Conjunct Resolution in the Face of Verbal Omissions

Verbal omissions are complex syntactic phenomena in VP coordination structures. They occur when verbs and (some of) their arguments are omitted from subsequent clauses after being explicitly stated in an initial clause. Recovering these omitted elements is necessary for accurate interpretation of the sentence, and while humans easily and intuitively fill in the missing information, state-of-the-art models continue to struggle with this task. Previous work is limited to small-scale datasets, synthetic data creation methods, and to resolution methods in the dependency-graph level. In this work we propose a conjunct resolution task that operates directly on the text and makes use of a split-and-rephrase paradigm in order to recover the missing elements in the coordination structure. To this end, we first formulate a pragmatic framework of verbal omissions which describes the different types of omissions, and develop an automatic scalable collection method. Based on this method, we curate a large dataset, containing over 10K examples of naturally-occurring verbal omissions with crowd-sourced annotations of the resolved conjuncts. We train various neural baselines for this task, and show that while our best method obtains decent performance, it leaves ample space for improvement. We propose our dataset, metrics and models as a starting point for future research on this topic.

==> background.tex <==
\section{Background} 
We focus on a specific type of coordination known as VP omission, which utilizes the parallel nature of coordinated clauses to omit repeating verb phrases in order to create a more concise and efficient structure. Here we provide background on the different sub-cases: we examine two types of omission: middle omission (also known as gapping) and left omission. We also explore three types of complements that can occur in VP omissions: direct object, prepositional, and infinitive marker. Each combination of these omissions and complements results in distinct linguistic phenomena that we cover.

\paragraph{Coordination} sentences are composed of two or more clauses joined by a conjunction. These clauses are typically parallel in structure and syntactic type, such as both being VPs. An example of a coordination sentence is "Bob received three points for a win and Alice received one point for a draw." In this sentence, the conjunction "and" coordinates the two verb clauses, which are parallel in structure. Coordination sentences are frequently used to express lists of items, actions, or events and can include multiple conjunctions, such as "and", "or", or "but" to signal the relationship between the clauses.

\subsection{Types of VP Omissions}
\royi{somewhere in this section, describe non-contig cases?}
VP omissions utilize the parallel nature of coordination sentences to omit repeating VPs  have already been mentioned. This results in a more concise and efficient language structure. There are several forms in which VP omissions can occur, which are described as follows:

\paragraph{Middle Omission (Gapping)} is a form of ellipsis in coordination sentences that omits a verb from a non-initial conjunct, after appearing in a previous clause. For example, in the sentence "Bob \textbf{received} three points for a win and Alice \_\_ one point for a draw" the verb "received" is omitted from the second clause, but is understood from the context. %An interesting case of middle omissions is non-contiguous omissions, where more information is missing than the VP\citep{sebastianGapping} \royi{not sure he is the one who deserves this}. For instance: "Cruise’s film \textbf{took} £515,000 \textbf{at UK box offices at the weekend}, and 22 Jump Street \_\_ £1.5million \_\_". Such cases are linear in resolution, that is, if "took" appears first, it will also be omitted first. 

\paragraph{Left Omission} is a relaxed version of middle omission, where the subject is omitted with the VP. This is permitted when the subject is repeated across clauses. To illustrate, in the sentence "\textbf{The team received} three points for a win and \_\_ one point for a draw", "the team received" is omitted from the second clause, but is understood from the context.

\paragraph{Types of Complements}
We distinguish among three types of complements in VP Omissions: direct object, prepositional, and infinitive marker. Each resulting in a different phenomenon. Here we show each complement in both cases, middle omission and left omission.

\paragraph{Object Complement} is the standard case, where a direct object is the complement. Both examples (\labelcref{graph:jane_water}) and (\labelcref{graph:brown_dark}) in the introduction are cases of middle omissions with an object complement.
\begin{itemize}
     \item Middle Omission: Josh \textbf{likes} wine and Jane \_\_ water.
     \item Left Omission: \textbf{It sparked} dozens of comments and \_\_ loads of new ideas.
\end{itemize}

\paragraph{Prepositional Complement} is characterized by a "hanging" preposition in the clause containing the omission. For example, consider examples of middle omissions and left omissions:
\begin{itemize}
     \item Middle Omission: Josh \textbf{is working} from home and Mary \_\_ from the office.
     \item Left Omission:  \textbf{The goal is} worthy and \_\_ in sight.
\end{itemize}

\paragraph{Infinitive Marker Complement} is similar to the prepositional complement case, but instead, an infinitive marker is "hanging". The middle omission case creates an intriguing case in which an infinitive marker is immediately followed by a verb can be followed by another infinitive marker and a verb. This pattern can be continued indefinitely, to form an indefinitely long omission \citep{Ross1967aGapping}. To illustrate this, consider "I want to try to begin to write a novel and Mary \_\_ a play". To fully resolve this sentence, multiple connected verbs must be added to the second clause, specifically, "wants to try to begin to write", as can be seen in example (1).

\begin{itemize}
    \item Middle Omission: I \textbf{want to try to begin to write} a novel and
       \begin{enumerate}
        \renewcommand*\labelenumi{(\alph{enumi})}
         \item Mary \_\_ a play.
         \item Mary \_\_ to write a play.
         \item Mary \_\_ to begin to write a play.
         \item Mary \_\_ to try to begin to write a play.
        \end{enumerate}
    \item Left Omission: \textbf{Minaj declined} to have photos taken or \_\_ to file a complaint, police said.
\end{itemize}




% \paragraph{Classic Gapping} refers to the linguistics definition, in which a verb that has been used in an initial clause is omitted from subsequent clauses, while the verb's subject and object remain. This construction is well-described in linguistics literature. As an example, in (\labelcref{graph:jane_water}), the second clause "Jane \_\_ water" contains a gap between "Jane" and "water". Another instance of this construction can be seen in (\labelcref{graph:brown_dark}) \royi{do we need to refer to the example in the gapping sub-section above too?}.

% \paragraph{Subject Verb Gapping} is a phenomenon similar to classic gapping, but with the additional omission of the subject. This construction is only applicable in cases where the subject remains constant across clauses. For instance, in the sentence "[It sparked]\textsubscript{anc} dozens of comments and \_\_ loads of new ideas", the subject "it" applies to both clauses, but is only explicitly mentioned in the first clause, in similar fashion to the verb "sparked". %Its dependency graph \royi{add here} shows a conjunction relation between "dozens" and "loads", instead of two verbs, indicating the lack of self-sufficiency in the second clause.

% % \begin{enumerate}
% %     \renewcommand*\labelenumi{(\theenumi)} 
% %         \setcounter{enumi}{3}
% %     \item \input{graphs/loads_of_new_ideas.tex}
% % \end{enumerate}

% \paragraph{Prepositional Gapping} is characterized by the omission of a VP in a non-initial clause, resulting in a "hanging" preposition. For example, in the sentence "[The goal is]\textsubscript{anc} worthy and \_\_ in sight", the gap causes the preposition "in" to become the head of the gapped clause, leading to an awkward interpretation of the sentence in which the conjunct relation (\textit{conj}) is between an adjective ("worthy") and a preposition ("in") rather than between the verbs, which would be the case if the verb had not been omitted.

% \begin{enumerate}
%     \renewcommand*\labelenumi{(\theenumi)} 
%         \setcounter{enumi}{3}
%     \item \input{graphs/worthy_and_in_sight.tex}
% \end{enumerate}

% % show case of dependency graph and how it changes the graph

% \paragraph{Verb Cluster Gapping} is similar to the prepositional gapping case, but instead, an infinitive marker is left "hanging". This creates an intriguing sub-case, in which an infinitive marker that is immediately followed by a verb can be followed by another infinitive marker and a verb. This pattern can be continued indefinitely, to form an infinitely long gap \citep{Ross1967aGapping}. To illustrate this, consider "[I want to try to begin to write]\textsubscript{anc} a novel and Mary \_\_ a play". To fully resolve this sentence, multiple connected verbs must be added to the second clause, specifically, "want to try to begin to write", as can be seen in example (5).

% % Try to create this figure across a page but with its reconstruction and dotted edges to show its complete for and where edges would change...

% % \begin{enumerate}
% %     \renewcommand*\labelenumi{(\theenumi)} 
% %         \setcounter{enumi}{4}
% %     \item \input{graphs/mary_a_play.tex}
% % \end{enumerate}

% \begin{enumerate}
%     \renewcommand*\labelenumi{(\theenumi)}
%     \setcounter{enumi}{4}
%     \item I want to try to begin to write a play and
%        \begin{enumerate}
%          \item … Mary \_\_ a play.
%          \item … Mary \_\_ to write a play.
%          \item … Mary \_\_ to begin to write a play.
%          \item … Mary \_\_ to try to begin to write a play.
%      \end{enumerate}
% \end{enumerate}



==> baselines.tex <==
\section{Experiments}
In order to establish a benchmark for our proposed task, we implement a set of baselines to compare against. These baselines represent commonly used techniques in the field and serve as a point of reference for our results. In this section, we describe these baselines in detail and provide an analysis of their performance on our dataset.

We fine-tune T5-small, T5-large \citep{t5}, and test few-shot inference on the most up to date GPT-3\footnote{text-davinci-003} \citep{gpt3}.
\subsection{Fine-Tuning Set Up}
\subsection{Few-Shot Inference Set Up}
\subsection{Evaluation Metric}
\subsection{Results}

\input{tables/baseline_table.tex}

\subsection{Error Analysis}
% \subsection{Identification Baseline}
% This can also be framed as a multiclass classification problem, where the label space consists of: \textit{\{and, or, but, symmetric\}}, where \textit{symmetric} marks no violation occurred for that conjunction, and the other labels mark the conjunction that violates the symmetry. 
 
% This can also be framed as a multiclass classification problem, where the label space is: \textit{\{and, or, but, None\}}, where \textit{None} marks no violation occurred for that conjunction, and the other labels mark the conjunction that violates the symmetry.


==> tables/dataset_sentences_stats.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|r|r|r}
Split & Num Sentences & Num Splittable Sentences  \\ 
\hline
Train  & 8,166 &  b\\
Validation & 1,021 & b\\
Test &  1,019 & b\\
\hline
All &  10,206 & b \\
% Avg num of missing verbs per sentence & 2.14 \\ 
\end{tabular}
\caption{Sentences Statistics}
\label{tab:dataset_sentences_stats}
\end{table}
